"Observing and Analyzing" Images From a Simulated High Redshift Universe

We investigate the high-redshift evolution of the restframe UV-luminosity function (LF) of galaxies via hydrodynamical cosmological simulations, coupled with an emulated observational astronomy pipeline that provides a direct comparison with observations. We do this by creating mock images and synthetic galaxy catalogs of approximately 100 square arcminute fields from the numerical model at redshifts ~ 4.5 to 10.4. We include the effects of dust extinction and the point spread function (PSF) for the Hubble WFC3 camera for comparison with space observations. We also include the expected zodiacal background to predict its effect on space observations, including future missions such as the James Webb Space Telescope (JWST). When our model catalogs are fitted to Schechter function parameters, we predict that the faint-end slope alpha of the LF evolves as alpha = -1.16 - 0.12 z over the redshift range z ~ 4.5 to 7.7, in excellent agreement with observations from e.g., Hathi et al. (2010). However, for redshifts z ~ 6 to 10.4, alpha(z) appears to display a shallower evolution, alpha = -1.79 - 0.03 z. Augmenting the simulations with more detailed physics - specifically stellar winds and supernovae (SN) - produces similar results. The model shows an overproduction of galaxies, especially at faint magnitudes, compared with the observations, although the discrepancy is reduced when dust extinction is taken into account.

==> Overview.tex <==
%
The luminosity function (LF) of galaxies is an important indicator of galaxy
assembly and evolution. It traces the star-formation rate (SFR) and contains 
clues to merger rates and other physical processes, such as feedback from
supernovae (SN) and active galactic nuclei (AGN). 
Numerical simulations --- essential to understanding and predicting
the highly non-linear processes in large scale structure formation ---
are often difficult to interpret with respect to the actual astronomical 
observations. This is due to many factors, including the effect of noise, 
such as the sky-background. 
It is thus difficult to draw precise inferences 
between the numerical predictions of the model and
the images actually observed in astronomy.  Overzier et al. (2013) 
characterized the problem of the current state of the relation between theory 
and observation as being mostly one-directional, in that ``physical quantities 
estimated from observations were compared with theoretical predictions,''
and that the interpretation needed to also be done from the other direction. 


To help bridge this gap between theory and observations, 
we extend the model to include simulation of the observational pipeline. 
That is, we form images from the simulations of galaxy formation,
using the stellar population
synthesis models of Bruzual \& Charlot (2003, hereafter BC03)  
to predict the observed stellar light distributions, and 
process these  to create mock galaxy catalogs using Source Extractor
(``SExtractor''; Bertin \& Arnouts 1996).


Overzier et al. (2013) summarized previous work done in this area, 
such as Bouwens et al. 1999, who coupled galaxy evolution 
models to SED models to predict luminosities at high redshifts, 
and Bouwens, Illingworth \& Magee (2006), who predicted the
evolution of galaxy properties by artificially redshifting selected galaxy
images, producing new synthetic images.  Overzier, et al. (2013) also discuss 
producing ``observed'' image sets from semi-analytic models (SAMs).


In this work, we use gas and hydrodynamic models based on Gadget2 
(Springel (2000); Springel et al. 2001; Springel \& Hernquist  2003), 
including star-formation.  Overzier et al. (2013) point out that 
hydrodynamical simulations with dark matter (DM), gas and stars have been used 
(e.g., Jonsson et al. 2006; Lotz et al. 2008, 2010; Robertson \& Bullock 2008; 
Wuyts et al. 2009, and Chiliangarian et al. 2010). 
However, these were mainly used to study the effects of dust
on the observations, and were not on cosmological scales. 

Realistic synthetic telescope images produced from the output of
hierarchical simulations to emulate sky surveys were generated by
Blaizot, et al. 2005. These were also done by using the output of SAMs,
processing the results of DM halo simulations. They used methods
similar to those used here, in terms of the use of translation and rotation
of multiple slices of data at different redshifts
to produce artificial images and catalogs. 
Also, Nagamine (2007) coupled cosmological hydrodynamic CDM models to
population synthesis models to predict galaxy properties, though he did not
produce image sets. 

The use of hydrodynamic numerical simulations limits our ability to 
reproduce survey-size scales of many square degrees over cosmological 
time scales, since we do not use transverse replication as in Blaizot et al. 
(2005). However, we are able to produce images on Great Observatories
Origins Deep Surveys (GOODS) mosaics fields of 
8 -- 10 arcminutes with HST and in the future with JWST at redshifts of 
$z \simeq 4.5 $ to 11. While it is true, as Overzier et al. (2013) point out, 
that it is time consuming to run hydrodynamic simulations
with different sets of parameter values, we feel it is crucial to perform
these simulations with minimal assumptions, to see how well we can reproduce 
the actual observations with physics-based model inputs. This also aids in
deducing the effects of different physics on the outcome, as these can be
added to the model.  This was also done by Haas (2010), who used 
hydrodynamic simulations from the OverWhelmingly Large Simulations
(Schaye et al. 2010) to study the LF's of mock galaxies, though this work
was in the $K$-- and $B$--  band filters and confined to lower redshifts, $z  <  4$.


Overzier et al. (2013) pursued a similar approach in the ``Millennium Run
Observatory'' (MROB), using semi-analytical models.  
They implemented a rich user-interface for perusing
the simulation data-base at different wavelengths and filters, and 
included a number of observational artifacts. 
Our work is more focussed on 
predicting the faint-end luminosity function of galaxies, something that is
of considerable interest to observers and relevant to the direct planning
of missions such as JWST. The results presented here can thus potentially
be used to guide the planning of future JWST observations.


